Demographic Bias: A Challenge for Fingervein Recognition Systems?

Recently, concerns regarding potential biases in the underlying algorithms of many automated systems (including biometrics) have been raised. In this context, a biased algorithm produces statistically different outcomes for different groups of individuals based on certain (often protected by anti-discrimination legislation) attributes such as sex and age. While several preliminary studies investigating this matter for facial recognition algorithms do exist, said topic has not yet been addressed for vascular biometric characteristics. Accordingly, in this paper, several popular types of recognition algorithms are benchmarked to ascertain the matter for fingervein recognition. The experimental evaluation suggests lack of bias for the tested algorithms, although future works with larger datasets are needed to validate and confirm those preliminary results.

==> performance.tex <==
\begin{tabular}{lll}
\toprule
Dataset & Algorithm & EER (in \%) \\
\midrule
MMCBNU & LCNN & 2.2 \\
& LBP & 1.3 \\
& MC & 1.8 \\
& PC & 1.7 \\
& SIFT & 2.0 \\
\midrule
PLUS & LCNN & 4.5 \\
& LBP & 3.6 \\
& MC & 0.5 \\
& PC & 0.2 \\
& SIFT & 0.8 \\
\midrule
UTFVP & LCNN & 7.0\\
& LBP & 1.5 \\
& MC & 0.2 \\
& PC & 0.4 \\
& SIFT & 1.5 \\
\midrule
VERA & LBP & 3.2 \\
& MC & 1.8 \\
& PC & 2.3 \\
& SIFT & 2.6 \\
\bottomrule
\end{tabular}

